Neutrino-heated winds from rotating proto-magnetars

We calculate the steady-state properties of neutrino-driven winds from strongly magnetized, rotating proto-neutron stars (`proto-magnetars') under the assumption that the outflow geometry is set by the force-free magnetic field of an aligned dipole. Our goal is to assess proto-magnetars as sites of r-process nucleosynthesis and gamma-ray burst engines. One dimensional solutions calculated along flux tubes corresponding to different polar field lines are stitched together to determine the global properties of the flow at a given neutrino luminosity and rotation period. Proto-magnetars with rotation periods of P~2-5 ms are shown to produce outflows more favorable for the production of third-peak r-process nuclei due to their much shorter expansion times through the seed nucleus formation region, yet only moderately lower entropies, as compared to normal spherical PNS winds. Proto-magnetars with moderately rapid birth periods P~3-5 ms may thus represent a promising Galactic r-process site which is compatible with a variety of other observations, including the recent discovery of possible magnetar-powered supernovae in metal poor galaxies. We also confirm previous results that the outflows from proto-magnetars with P~1-2 ms can achieve maximum Lorentz factors Gamma ~ 100-1000 in the range necessary to power gamma-ray bursts (GRBs). The implications of GRB jets with a heavy nuclei-dominated composition as sources of ultra-high energy cosmic rays are also addressed.

==> l12_02.0_33_1.0e+52.tex <==
$2^\star$ & $10^\star$ & $1.5^\star$ & $1.1\cdot 10^{-2}$ & $29^\star$ & $0.5^\star$ & $0.4298^\star$ & $8.4^\star$ & $36^\star$ & $2.2\cdot 10^{0}$ & $0.4^\star$\\


==> l12_03.0_22_1.0e+52.tex <==
$3^\star$ & $10^\star$ & $1.1^\star$ & $4.8\cdot 10^{-3}$ & $39^\star$ & $0.9^\star$ & $0.4448^\star$ & $9.9^\star$ & $42^\star$ & $2.5\cdot 10^{-1}$ & $0.5^\star$\\


==> l12_04.0_28_1.0e+52.tex <==
$4^\star$ & $10^\star$ & $1.6^\star$ & $4.8\cdot 10^{-3}$ & $41^\star$ & $1.0^\star$ & $0.4456^\star$ & $9.8^\star$ & $42^\star$ & $7.1\cdot 10^{-1}$ & $0.6^\star$\\


==> l12_05.0_24_1.0e+52.tex <==
$5^\star$ & $10^\star$ & $1.5^\star$ & $4.1\cdot 10^{-3}$ & $45^\star$ & $1.4^\star$ & $0.4477^\star$ & $8.9^\star$ & $46^\star$ & $4.5\cdot 10^{-1}$ & $0.7^\star$\\


==> res_02.0_33_1.0e+52.tex <==
$2^\circ$ & $10^\circ$ & $1.5^\circ$ & $1.1\cdot 10^{-2}$ & $29^\circ$ & $0.5^\circ$ & $0.4298^\circ$ & $8.4^\circ$ & $36^\circ$ & $2.2\cdot 10^{0}$ & $0.4^\circ$\\


==> res_02.0_41_1.0e+52.tex <==
$2^\star$ & $10^\star$ & $1.8^\star$ & $1.5\cdot 10^{-2}$ & $25^\star$ & $0.5^\star$ & $0.4212^\star$ & $5.6^\star$ & $32^\star$ & $1.0\cdot 10^{1}$ & $0.5^\star$\\


==> res_03.0_22_1.0e+52.tex <==
$3^\circ$ & $10^\circ$ & $1.1^\circ$ & $4.8\cdot 10^{-3}$ & $39^\circ$ & $0.9^\circ$ & $0.4448^\circ$ & $9.9^\circ$ & $42^\circ$ & $2.5\cdot 10^{-1}$ & $0.5^\circ$\\


==> res_03.0_33_1.0e+52.tex <==
$3^\star$ & $10^\star$ & $1.7^\star$ & $6.5\cdot 10^{-3}$ & $35^\star$ & $0.7^\star$ & $0.4412^\star$ & $10.3^\star$ & $38^\star$ & $1.6\cdot 10^{0}$ & $0.4^\star$\\

